Software solutions for form-based collection of data and the semantic enrichment of form data

Data collection is an important part of many citizen science projects as well as other fields of research, particularly in life sciences. Mobile applications with form-based surveys are increasingly used to support this, due to the large number of mobile devices and their growing number of built-in sensors. Since the composition of form-based surveys from scratch can be a tedious task, multiple tools have been published that can help with their design and distribution as well as the data collection via mobile devices and the data storage. Some even support simple data analysis. With this increasing number of software options project leaders will often face the question, which tool is most suitable for their current use case. With that in mind, this project pursues two main objectives: 1. To present an overview of a selection of survey design tools and their capabilities in order to provide a clear foundation for such a decision. 2. To examine if any tool provides the capability to collect and export data in a way that can easily be used and interpreted by other applications or persons. This aspect includes the supply of metadata about the data collection process and the data itself, information about the meaning of the data as well as an export format that can easily be processed.

==> Chapters/features.tex <==
\rowcolors{2}{gray!25}{white}
\begin{tabu} to \linewidth{X[3,r,m]|X[1,m,c]X[1,m,c]X[1,m,c]X[1,m,c]X[1,m,c]X[1,m,c]X[1,m,c]} 
\rowcolor{gray!50}
\strut  & \strut EpiCollect 5 & \strut ODKv1 & \strut ODKv2 & \strut Kobo & \strut Ohmage & \strut SurveyCTO & \strut Magpi \\ 
\hline 
Form Designer & \strut \cmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark \\ 
Skip Logic & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark \\ 
Localization & \strut \xmark & \strut \cmark & \strut \cmark & \strut \omark & \strut \xmark & \strut \cmark & \strut \xmark \\ 
Calculations & \strut \xmark & \strut \cmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \cmark & \strut \cmark \\ 
Queries & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
Linked Tables & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
Required \& Optional Fields & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark \\ 
Validation & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark \\ 
Xform Export & \strut \xmark & \strut \omark & \strut \xmark & \strut \omark & \strut \xmark & \strut \omark & \strut \xmark \\ 
Xform Import & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \omark & \strut \cmark \\ 
XLSForm Export & \strut \xmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \xmark \\ 
XLSForm Import & \strut \xmark & \strut \xmark & \strut \cmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \xmark \\ 
CSV Export & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark \\ 
JSON Export & \strut \cmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
XLS Export & \strut \xmark & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \cmark \\ 
XML Export & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
XML/KML Export & \strut \xmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark \\ 
RDF Export & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
Active Development & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \cmark \\ 
License & \strut - & \strut Apache\footnote{Apache License 2.0} & \strut Apache\footnote{Apache License 2.0} & \strut GNU Af\footnote{GNU Affero General Public License v3.0 \& Apache License 2.0} & \strut Apache\footnote{Apache License 2.0} & \strut - & \strut - \\ 
Open Source & \strut \xmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \xmark & \strut \xmark \\ 
Self-hosting & \strut \xmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \xmark & \strut \xmark \\ 
Data encryption & \strut \xmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \cmark & \strut \xmark \\ 
Semantic Enrichment & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
HXL support & \strut \xmark & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
Building custom prompts & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \xmark \\ 
Visualization/Data management on mobile device & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \omark \\ 
Offline-Collection & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark \\ 
Android App & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark & \strut \cmark \\ 
iOS App & \strut \cmark & \strut \xmark & \strut \xmark & \strut \xmark & \strut \cmark & \strut \xmark & \strut \cmark \\ 
 \end{tabu}
